Scaling Motion Planning Infeasibility Proofs

Achieving completeness in the motion planning problem demands substantial computation power, especially in high dimensions. Recent developments in parallel computing have rendered this more achievable. We introduce an embarrassingly parallel algorithm for constructing infeasibility proofs. Specifically, we design and implement a manifold triangulation algorithm on GPUs based on manifold tracing with Coxeter triangulation. To address the challenge of extensive memory usage within limited GPU memory resources during triangulation, we introduce batch triangulation as part of our design. The algorithm provides two orders of magnitude speed-up compared to the previous method for constructing infeasibility proofs. The resulting asymptotically complete motion planning algorithm effectively leverages the computational capabilities of both CPU and GPU architectures and maintains minimum data transfer between the two parts. We perform experiments on 5-DoF and 6-Dof manipulator scenes.

==> alg/construct.tex <==
\begin{algorithm}
  \KwIn{$Ls$\tcp*[l]{Line segments}}
  \KwIn{$Ps$\tcp*[l]{Line to intersection map}}
  \KwOut{$T$\tcp*[l]{Triangulation of manifold}}
   $M \leftarrow \{\}$ \tcp*[l]{Concurrent hash
     table}\label{line:hashtable}
  \Pragma{parallel for}
    \ForEach %(\tcp*[h]{sample in parallel})\
    {$l \in Ls$}
    {\label{line:eachline}
    \ForEach %(\tcp*[h]{sample in parallel})
    {$c \in l.\FuncSty{coface}(n)$} {
    $M[c].\FuncSty{add}(Ps[l])$\label{line:add1}\;
    % \eIf{$Ps[l] \in \CObs$}{
    % $M[c].\FuncSty{add}(Ps[l])$\label{line:add1}\;
    % }{
    % $ p_{new} \leftarrow \FuncSty{Elastic-Update}(Ps[l])$\label{line:localfix}\;
    % \eIf
    % (\tcp*[h]{Elastic-Update succeeds})
    % {$p_{new}$}{$M[c].\FuncSty{add}(p_{new})$\label{line:add2}\;}(\tcp*[h]{Elastic-Update fails})
    % {\Return}
    % }
    }
    }

    $T \leftarrow \FuncSty{collect-values-for-each-key}(M)$\;

% \ForEach
% {$t \in T$}{\label{line:tinT}
% \If{$|t| > n$}{
% $ts \leftarrow \FuncSty{decompose}(t)$\label{line:decompose}\;
% $T.\FuncSty{remove}(t)$\;
% $T.\FuncSty{add}(ts)$\label{line:add-decompose}\;
% }
% }

  \caption{Construct Triangulation}
  \label{alg:construct}
\end{algorithm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../report.tex"
%%% End:


==> alg/intersection.tex <==
\begin{algorithm}
  \KwIn{$\MF(\conf)$\tcp*[l]{Manifold function}}
  \KwIn{$\vone, \vtwo$\tcp*[l]{Line segment vertices}}
  \KwOut{$\vp$\tcp*[l]{Intersection Point}}

  \Repeat( \tcp*[h]{False-Position~\cite{ninechapters,conte2017elementary}})
  {$|\MF(\vp)| < \tau$}
  {

  %$\lambda_1 \leftarrow \MF(\vtwo)/(\MF(\vtwo) - \MF(\vone))$\;
  %$\lambda_2 \leftarrow \MF(\vone)/(\MF(\vone) - \MF(\vtwo))$\;
  %$\vp \leftarrow \lambda_1 \vone + \lambda_2 \vtwo$\;
  $\vp \leftarrow \frac{\vone \MF(\vtwo) - \vtwo \MF(\vone)}
                       {\MF(\vtwo) - \MF(\vone)}$\;
                       % \tcp*[l]{False Position~\cite{conte2017elementary}}

  \lIf{$\MF(\vp) * \MF(\vone) > 0$ }
  {$\vtwo \leftarrow p$}
   \lElse{$\vone \leftarrow \vp$}

  }( \tcp*[h]{within tolerance $\tau$})
  \caption{Calculate Intersection Point}
  \label{alg:inter}

\end{algorithm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../report.tex"
%%% End:


==> alg/leanring_sampling.tex <==
\begin{algorithm}
  \KwIn{$G$\tcp*[l]{Planning Graph}}
  \KwIn{$\Qobs$\tcp*[l]{Set of $\CObs$ configurations}}
  \KwOut{$G$, $\Qseeds$\tcp*[l]{Planning Graph}}

  \Repeat()
  {\FuncSty{Timeout} $or$ \FuncSty{Found path} $or$ \FuncSty{Found inf}}
  {
  $\Qseeds \leftarrow \emptyset $\;
  $Q \leftarrow \{q | q \in G\} + \Qobs $\label{line:Q}\;
  $\Pstart, \Pgoal$ $\leftarrow$ $\FuncSty{Acquire-Input-Data}(G)$\label{line:inputdata}\;
  $f$ $\leftarrow \FuncSty{train-SVM}(\Pstart, \Pgoal)$\label{line:train}\;
    \Pragma{parallel for}
    \ForEach %(\tcp*[h]{sample in parallel})
    {$\conf \in Q$}
    {
      $\qman \leftarrow \FuncSty{sample-manifold}(\conf, f)$\label{line:sample}\;
        \If{$\qman \in \CFree$} {
          $\FuncSty{add-sample}(G, \qman)$\label{line:addstartgoal}\;
        }
      $\Qseeds \FuncSty{.add}(\qman)$\label{line:seeds}\;
    }
  }
  \caption{SDCL}
  \label{alg:sdcl}
\end{algorithm}



==> alg/local_update.tex <==
\begin{algorithm}
  \KwIn{$G$\tcp*[l]{Planning Graph}}
  \KwIn{$\conf$\tcp*[l]{Point in $\CFree$}}
  \KwIn{$F(\conf)$\tcp*[l]{Up-to-Date Manifold}}
  \KwOut{$G$, $F$, $\conf$\tcc*[l]{Planning Graph, New Manifold, New Point}}
$\FuncSty{add-sample}(G, \conf)$\label{line:toG1}\;
\Loop {
   $\conf \leftarrow \FuncSty{project-to-manifold}(\conf, F)$\label{line:sample}\;
\lIf{$\conf \in \CObs$ $or$ $\conf = \emptyset$} {\Return}
$\FuncSty{add-sample}(G, \conf)$\label{line:toG}\;
  $\Pstart, \Pgoal$ $\leftarrow$ $\FuncSty{Acquire-Input-Data}(G)$\label{line:inputdata}\;
  $F$ $\leftarrow \FuncSty{train-SVM}(\Pstart, \Pgoal)$\label{line:retrain}\;
}

  % \Repeat()
  % {$\conf \in \CObs$ $or$ $\conf = \emptyset$}
  % {
  % $\FuncSty{add-sample}(G, \conf)$\label{line:toG}\;
  %  $\conf \leftarrow \FuncSty{sample-manifold}(\conf, F)$\label{line:sample}\;

  % $\Pstart, \Pgoal$ $\leftarrow$ $\FuncSty{Acquire-Input-Data}(G)$\label{line:inputdata}\;
  % $F$ $\leftarrow \FuncSty{train-SVM}(\Pstart, \Pgoal)$\label{line:retrain}\;
  % }
  \caption{Elastic-Update}
  \label{alg:local}
\end{algorithm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../report.tex"
%%% End:


==> alg/manifold_tracing.tex <==
\begin{algorithm}
  \KwIn{$\Tri$\tcp*[l]{$\Re^n$ Coxeter triangulation}}
  \KwIn{$F(\conf)$\tcp*[l]{Up-to-Date manifold}}
  \KwIn{$\Qseeds$\tcp*[l]{Seed points on manifold}}
  \KwOut{$Ls$\tcp*[l]{Intersecting line segs}}
  $Q \leftarrow \emptyset$\tcp*[l]{Empty queue for line segs}
    \Pragma{parallel for}
  \ForEach
    {$\conf \in \Qseeds$}{
    $ls \leftarrow \FuncSty{locate}(\conf)$\tcp*[l]{locate starting simplex, return its line segments}
    $Q.\FuncSty{add}(ls)$\;
    $Ls.\FuncSty{add}(ls)$\;
    }
  \Pragma{parallel for}
  \Repeat{$Q = \emptyset$}
  {
  $ls \leftarrow Q.\FuncSty{pop}()$\;
  \ForEach
    {$c \in ls.\FuncSty{coface}(2)$} {
    \ForEach
    {$l \in c.\FuncSty{face}(1)$}{
    \If{$l \notin Ls$ \& $l~\FuncSty{intersects}~F$}{
    $Q.\FuncSty{add}(l)$\;
    $Ls.\FuncSty{add}(l)$\;
    }
    }
    }
  }


  \caption{Parallel Manifold Tracing}
  \label{alg:mani-tracing}
\end{algorithm}
